Online Continual Learning for Embedded Devices

Real-time on-device continual learning is needed for new applications such as home robots, user personalization on smartphones, and augmented/virtual reality headsets. However, this setting poses unique challenges: embedded devices have limited memory and compute capacity and conventional machine learning models suffer from catastrophic forgetting when updated on non-stationary data streams. While several online continual learning models have been developed, their effectiveness for embedded applications has not been rigorously studied. In this paper, we first identify criteria that online continual learners must meet to effectively perform real-time, on-device learning. We then study the efficacy of several online continual learning methods when used with mobile neural networks. We measure their performance, memory usage, compute requirements, and ability to generalize to out-of-domain inputs.

==> tables/compute_time.tex <==
\begin{table}[t]
\caption{Run times in minutes for each online continual learner when trained and evaluated on the OpenLORIS dataset with the low-shot instance ordering. All models were evaluated on the same hardware (i.e., desktop computer with a Titan XP GPU and 128 GB of RAM). \label{tab:compute}}
\centering
% \resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textsc{Model} & \textsc{MNet-S} & \textsc{MNet-L} & \textsc{ENet-B0} & \textsc{ENet-B1} & \textsc{RN-18} \\ 
\midrule
Perceptron & & & & & \\
Fine-Tune & 18.2 & 18.9 & 20.9 & 26.3 & 18.7 \\
Naive Bayes & 22.0 & 23.2 & 25.9 & 30.0 & 23.0 \\
SOvR & 21.9 & 23.0 & 25.1 & 29.2 & 22.7 \\
NCM & 18.0 & 18.8 & 20.9 & 26.2 & 18.7 \\
Replay (2pc) & 18.3 & 19.1 & 21.2 & 26.6 & 19.0 \\
Replay (20pc) & 18.3 & 19.1 & 21.2 & 26.5 & 18.8 \\
SLDA & 18.1 & 18.9 & 21.0 & 26.4 & 18.7 \\
\bottomrule
\end{tabular}
% }
\end{table}

==> tables/datasets.tex <==
\begin{table}[t]
\caption{Dataset Statistics  \label{tab:dataset-stats}}
\centering
% \resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textsc{Statistic} & \textsc{Places-365} & \textsc{Places-LT} & \textsc{OpenLORIS} \\ 
\midrule
\# Classes & 365 & 365 & 40 \\
\# Train Samples & 1803460 & 62500 & 440919 \\
Min Train Samples Per Class & 3068 & 5 & 2472 \\
Max Train Samples Per Class & 5000 & 4980 & 22248 \\
\# Test Samples & 36500 & 36500 & 53295 \\
Min Test Samples Per Class & 100 & 100 & 288 \\
Max Test Samples Per Class & 100 & 100 & 2592 \\
Image Type & Static & Static & Video \\
\bottomrule
\end{tabular}
% }
\end{table}

==> tables/memory.tex <==
\begin{table}[t]
\caption{Memory requirements for each architecture and online continual learning model in MB for a 365 category dataset. Note that the online continual learners would also need to store the network architecture. \label{tab:memory}}
\centering
% \resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textsc{Model} & \textsc{MNet-S} & \textsc{MNet-L} & \textsc{ENet-B0} & \textsc{ENet-B1} & \textsc{RN-18} \\ 
\midrule
Backbone Size & 3.7 & 11.9 & 16.0 & 26.1 & 44.7 \\
\midrule 
Perceptron & 0.8 & 1.4 & 1.9 & 1.9 & 0.8 \\
Fine-Tune & 0.8 & 1.4 & 1.9 & 1.9 & 0.8 \\
Naive Bayes & 2.5 & 4.2 & 5.6 & 5.6 & 2.2 \\
SOvR & 0.8 & 1.4 & 1.9 & 1.9 & 0.8 \\
NCM & 0.8 & 1.4 & 1.9 & 1.9 & 0.8 \\
Replay (2pc) & 2.5 & 4.2 & 5.6 & 5.6 & 2.2 \\
Replay (20pc) & 17.7 & 29.4 & 39.2 & 39.2 & 15.7 \\
SLDA & 2.2 & 5.1 & 8.4 & 8.4 & 1.8 \\
\bottomrule
\end{tabular}
% }
\end{table}

==> tables/train_vs_inference_times.tex <==
\begin{table}[t]
\caption{Ratio of train time versus inference time for each continual learner with each backbone CNN. \label{tab:compute-train-vs-inference}}
\centering
% \resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textsc{Model} & \textsc{MNet-S} & \textsc{MNet-L} & \textsc{ENet-B0} & \textsc{ENet-B1} & \textsc{RN-18} & \textsc{Mean} \\ 
\midrule
Perceptron & 9.2 & 9.5 & 10.2 & 9.1 & 9.4 & 9.5 \\
Fine-Tune & 11.3 & 12.0 & 12.2 & 11.6 & 10.4 & 11.5 \\
Naive Bayes & 1.9 & 2.3 & 2.0 & 2.1 & 2.4 & 2.1 \\
SOvR & 1.6 & 1.5 & 1.4 & 1.6 & 1.4 & 1.5 \\
CBCL & 3.6 & 3.4 & 3.6 & 3.6 & 3.4 & 3.5 \\
NCM & 3.2 & 3.2 & 3.1 & 3.1 & 3.2 & 3.2 \\
Replay (2pc) & 63.4 & 62.5 & 58.3 & 60.8 & 59.1 & 60.8 \\
Replay (20pc) & 62.5 & 60.3 & 59.3 & 62.6 & 58.0 & 60.5 \\
SLDA & 4.9 & 4.5 & 4.2 & 4.9 & 4.8 & 4.7 \\
\bottomrule
\end{tabular}
% }
\end{table}
